Listening for Expert Identified Linguistic Features: Assessment of Audio Deepfake Discernment among Undergraduate Students

This paper evaluates the impact of training undergraduate students to improve their audio deepfake discernment ability by listening for expert-defined linguistic features. Such features have been shown to improve performance of AI algorithms; here, we ascertain whether this improvement in AI algorithms also translates to improvement of the perceptual awareness and discernment ability of listeners. With humans as the weakest link in any cybersecurity solution, we propose that listener discernment is a key factor for improving trustworthiness of audio content. In this study we determine whether training that familiarizes listeners with English language variation can improve their abilities to discern audio deepfakes. We focus on undergraduate students, as this demographic group is constantly exposed to social media and the potential for deception and misinformation online. To the best of our knowledge, our work is the first study to uniquely address English audio deepfake discernment through such techniques. Our research goes beyond informational training by introducing targeted linguistic cues to listeners as a deepfake discernment mechanism, via a training module. In a pre-/post- experimental design, we evaluated the impact of the training across 264 students as a representative cross section of all students at the University of Maryland, Baltimore County, and across experimental and control sections. Findings show that the experimental group showed a statistically significant decrease in their unsurety when evaluating audio clips and an improvement in their ability to correctly identify clips they were initially unsure about. While results are promising, future research will explore more robust and comprehensive trainings for greater impact.

==> fulltables.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\begin{tabular}{|ll|l|lll|lll|lll|lll|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{Group}}                                                                           & \multirow{2}{*}{N} & \multicolumn{3}{l|}{All Clips}                                                                                  & \multicolumn{3}{l|}{Real Clips}                                                                                 & \multicolumn{3}{l|}{Fake Accuracy}                                                                              & \multicolumn{3}{l|}{Unsurity}                                                                                   \\ \cline{4-15} 
\multicolumn{2}{|l|}{}                                                                                                 &                    & \multicolumn{1}{l|}{Pre}  & \multicolumn{1}{l|}{Post} & \begin{tabular}[c]{@{}l@{}}Paired \\ Diff.\end{tabular} & \multicolumn{1}{l|}{Pre}  & \multicolumn{1}{l|}{Post} & \begin{tabular}[c]{@{}l@{}}Paired \\ Diff.\end{tabular} & \multicolumn{1}{l|}{Pre}  & \multicolumn{1}{l|}{Post} & \begin{tabular}[c]{@{}l@{}}Paired \\ Diff.\end{tabular} & \multicolumn{1}{l|}{Pre}  & \multicolumn{1}{l|}{Post} & \begin{tabular}[c]{@{}l@{}}Paired \\ Diff.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{All Students}}                                                                & C & 32                 & \multicolumn{1}{l|}{0.48} & \multicolumn{1}{l|}{0.52} & 0.04*                                                   & \multicolumn{1}{l|}{0.55} & \multicolumn{1}{l|}{0.65} & 0.1*                                                    & \multicolumn{1}{l|}{0.46} & \multicolumn{1}{l|}{0.49} & 0.03                                                    & \multicolumn{1}{l|}{0.13} & \multicolumn{1}{l|}{0.11} & -0.02                                                   \\ \cline{2-15} 
\multicolumn{1}{|l|}{}                                                                                             & E & 99                 & \multicolumn{1}{l|}{0.49} & \multicolumn{1}{l|}{0.5}  & 0.01                                                    & \multicolumn{1}{l|}{0.58} & \multicolumn{1}{l|}{0.6}  & 0.03                                                    & \multicolumn{1}{l|}{0.47} & \multicolumn{1}{l|}{0.47} & 0.00                                                    & \multicolumn{1}{l|}{0.13} & \multicolumn{1}{l|}{0.11} & -0.02*                                                  \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Female}}                                                                      & C & 7                  & \multicolumn{1}{l|}{0.37} & \multicolumn{1}{l|}{0.41} & 0.04                                                    & \multicolumn{1}{l|}{0.46} & \multicolumn{1}{l|}{0.61} & 0.14                                                    & \multicolumn{1}{l|}{0.35} & \multicolumn{1}{l|}{0.36} & 0.01                                                    & \multicolumn{1}{l|}{0.21} & \multicolumn{1}{l|}{0.25} & 0.04                                                    \\ \cline{2-15} 
\multicolumn{1}{|l|}{}                                                                                             & E & 28                 & \multicolumn{1}{l|}{0.46} & \multicolumn{1}{l|}{0.47} & 0.01                                                    & \multicolumn{1}{l|}{0.49} & \multicolumn{1}{l|}{0.57} & 0.08                                                    & \multicolumn{1}{l|}{0.45} & \multicolumn{1}{l|}{0.44} & -0.01                                                   & \multicolumn{1}{l|}{0.16} & \multicolumn{1}{l|}{0.11} & -0.05*                                                  \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Male}}                                                                        & C & 22                 & \multicolumn{1}{l|}{0.52} & \multicolumn{1}{l|}{0.56} & 0.05                                                    & \multicolumn{1}{l|}{0.61} & \multicolumn{1}{l|}{0.69} & 0.08                                                    & \multicolumn{1}{l|}{0.49} & \multicolumn{1}{l|}{0.53} & 0.04                                                    & \multicolumn{1}{l|}{0.1}  & \multicolumn{1}{l|}{0.07} & -0.03                                                   \\ \cline{2-15} 
\multicolumn{1}{|l|}{}                                                                                             & E & 69                 & \multicolumn{1}{l|}{0.51} & \multicolumn{1}{l|}{0.51} & 0.01                                                    & \multicolumn{1}{l|}{0.61} & \multicolumn{1}{l|}{0.62} & 0.01                                                    & \multicolumn{1}{l|}{0.48} & \multicolumn{1}{l|}{0.48} & 0.00                                                    & \multicolumn{1}{l|}{0.13} & \multicolumn{1}{l|}{0.11} & -0.02                                                   \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}English  First \\ Language\end{tabular}}}        & C & 23                 & \multicolumn{1}{l|}{0.46} & \multicolumn{1}{l|}{0.52} & 0.06*                                                   & \multicolumn{1}{l|}{0.52} & \multicolumn{1}{l|}{0.62} & 0.10                                                    & \multicolumn{1}{l|}{0.45} & \multicolumn{1}{l|}{0.49} & 0.05                                                    & \multicolumn{1}{l|}{0.14} & \multicolumn{1}{l|}{0.12} & -0.02                                                   \\ \cline{2-15} 
\multicolumn{1}{|l|}{}                                                                                             & E & 83                 & \multicolumn{1}{l|}{0.49} & \multicolumn{1}{l|}{0.50} & 0.01                                                    & \multicolumn{1}{l|}{0.59} & \multicolumn{1}{l|}{0.61} & 0.02                                                    & \multicolumn{1}{l|}{0.47} & \multicolumn{1}{l|}{0.47} & 0.00                                                    & \multicolumn{1}{l|}{0.14} & \multicolumn{1}{l|}{0.11} & -0.03*                                                  \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}English  Not \\First  Language\end{tabular}}}    & C & 7                  & \multicolumn{1}{l|}{0.54} & \multicolumn{1}{l|}{0.51} & -0.02                                                   & \multicolumn{1}{l|}{0.71} & \multicolumn{1}{l|}{0.71} & 0.00                                                    & \multicolumn{1}{l|}{0.49} & \multicolumn{1}{l|}{0.46} & -0.03                                                   & \multicolumn{1}{l|}{0.13} & \multicolumn{1}{l|}{0.12} & -0.01                                                   \\ \cline{2-15} 
\multicolumn{1}{|l|}{}                                                                                             & E & 12                 & \multicolumn{1}{l|}{0.50} & \multicolumn{1}{l|}{0.52} & 0.03                                                    & \multicolumn{1}{l|}{0.5}  & \multicolumn{1}{l|}{0.58} & 0.08                                                    & \multicolumn{1}{l|}{0.49} & \multicolumn{1}{l|}{0.51} & 0.01                                                    & \multicolumn{1}{l|}{0.14} & \multicolumn{1}{l|}{0.12} & -0.03                                                   \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Fluent in  Another \\ Language\end{tabular}}}    & C & 17                 & \multicolumn{1}{l|}{0.45} & \multicolumn{1}{l|}{0.48} & 0.03                                                    & \multicolumn{1}{l|}{0.51} & \multicolumn{1}{l|}{0.62} & 0.10                                                    & \multicolumn{1}{l|}{0.43} & \multicolumn{1}{l|}{0.44} & 0.01                                                    & \multicolumn{1}{l|}{0.17} & \multicolumn{1}{l|}{0.16} & -0.01                                                   \\ \cline{2-15} 
\multicolumn{1}{|l|}{}                                                                                             & E & 41                 & \multicolumn{1}{l|}{0.49} & \multicolumn{1}{l|}{0.49} & 0.00                                                    & \multicolumn{1}{l|}{0.56} & \multicolumn{1}{l|}{0.57} & 0.01                                                    & \multicolumn{1}{l|}{0.47} & \multicolumn{1}{l|}{0.46} & -0.01                                                   & \multicolumn{1}{l|}{0.15} & \multicolumn{1}{l|}{0.13} & -0.02                                                   \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Not Fluent in  \\Another Language\end{tabular}}} & C & 14                 & \multicolumn{1}{l|}{0.51} & \multicolumn{1}{l|}{0.57} & 0.05                                                    & \multicolumn{1}{l|}{0.61} & \multicolumn{1}{l|}{0.68} & 0.07                                                    & \multicolumn{1}{l|}{0.49} & \multicolumn{1}{l|}{0.54} & 0.05                                                    & \multicolumn{1}{l|}{0.10} & \multicolumn{1}{l|}{0.06} & -0.03                                                   \\ \cline{2-15} 
\multicolumn{1}{|l|}{}                                                                                             & E & 54                 & \multicolumn{1}{l|}{0.5}  & \multicolumn{1}{l|}{0.51} & 0.01                                                    & \multicolumn{1}{l|}{0.58} & \multicolumn{1}{l|}{0.62} & 0.04                                                    & \multicolumn{1}{l|}{0.48} & \multicolumn{1}{l|}{0.48} & 0.00                                                    & \multicolumn{1}{l|}{0.13} & \multicolumn{1}{l|}{0.10} & -0.02                                                   \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Computing \\ Major\end{tabular}}}                  & C & 21                 & \multicolumn{1}{l|}{0.5}  & \multicolumn{1}{l|}{0.53} & 0.03                                                    & \multicolumn{1}{l|}{0.55} & \multicolumn{1}{l|}{0.68} & 0.13*                                                   & \multicolumn{1}{l|}{0.48} & \multicolumn{1}{l|}{0.49} & 0.01                                                    & \multicolumn{1}{l|}{0.14} & \multicolumn{1}{l|}{0.10} & -0.03                                                   \\ \cline{2-15} 
\multicolumn{1}{|l|}{}                                                                                             & E & 75                 & \multicolumn{1}{l|}{0.49} & \multicolumn{1}{l|}{0.49} & 0.01                                                    & \multicolumn{1}{l|}{0.57} & \multicolumn{1}{l|}{0.6}  & 0.03                                                    & \multicolumn{1}{l|}{0.47} & \multicolumn{1}{l|}{0.47} & 0.00                                                    & \multicolumn{1}{l|}{0.14} & \multicolumn{1}{l|}{0.11} & -0.02                                                   \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Non-Computing\\ Major\end{tabular}}}            & C & 8                  & \multicolumn{1}{l|}{0.38} & \multicolumn{1}{l|}{0.49} & 0.11*                                                   & \multicolumn{1}{l|}{0.47} & \multicolumn{1}{l|}{0.53} & 0.06                                                    & \multicolumn{1}{l|}{0.35} & \multicolumn{1}{l|}{0.48} & 0.13                                                    & \multicolumn{1}{l|}{0.14} & \multicolumn{1}{l|}{0.15} & 0.01                                                    \\ \cline{2-15} 
\multicolumn{1}{|l|}{}                                                                                             & E & 17                 & \multicolumn{1}{l|}{0.51} & \multicolumn{1}{l|}{0.52} & 0.01                                                    & \multicolumn{1}{l|}{0.56} & \multicolumn{1}{l|}{0.56} & 0.00                                                    & \multicolumn{1}{l|}{0.5}  & \multicolumn{1}{l|}{0.51} & 0.01                                                    & \multicolumn{1}{l|}{0.12} & \multicolumn{1}{l|}{0.1}  & -0.02                                                   \\ \hline
\end{tabular}

\caption{Mean Paired Difference (in Accuracy of Clip Recognition) Between Pre and Post Survey Administrations \\ \text{*} means the paired difference was significant (<0.05 p-value in paired t-test).}
\label{table:table1}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]

\begin{tabular}{|cl|l|lll|lll|lll|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{Group}}                                                                 & \multicolumn{1}{c|}{\multirow{2}{*}{N}} & \multicolumn{3}{c|}{Accuracy All clips}                       & \multicolumn{3}{c|}{Real Accuracy}                            & \multicolumn{3}{c|}{Fake Accuracy}                            \\ \cline{4-12} 
\multicolumn{2}{|c|}{}                                                                                       & \multicolumn{1}{c|}{}                   & \multicolumn{1}{l|}{Pre}  & \multicolumn{1}{l|}{Post} & Diff. & \multicolumn{1}{l|}{Pre}  & \multicolumn{1}{l|}{Post} & Diff. & \multicolumn{1}{l|}{Pre}  & \multicolumn{1}{l|}{Post} & Diff. \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{All Students}}                                                      & C & 25                                      & \multicolumn{1}{l|}{0.46} & \multicolumn{1}{l|}{0.51} & 0.05* & \multicolumn{1}{l|}{0.53} & \multicolumn{1}{l|}{0.63} & 0.10* & \multicolumn{1}{l|}{0.44} & \multicolumn{1}{l|}{0.48} & 0.04  \\ \cline{2-12} 
\multicolumn{1}{|c|}{}                                                                                   & E & 79                                      & \multicolumn{1}{l|}{0.47} & \multicolumn{1}{l|}{0.49} & 0.02  & \multicolumn{1}{l|}{0.56} & \multicolumn{1}{l|}{0.6}  & 0.04  & \multicolumn{1}{l|}{0.45} & \multicolumn{1}{l|}{0.46} & 0.01  \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Females}}                                                           & C & 7                                       & \multicolumn{1}{l|}{0.37} & \multicolumn{1}{l|}{0.41} & 0.04  & \multicolumn{1}{l|}{0.46} & \multicolumn{1}{l|}{0.61} & 0.14  & \multicolumn{1}{l|}{0.35} & \multicolumn{1}{l|}{0.36} & -0.01 \\ \cline{2-12} 
\multicolumn{1}{|c|}{}                                                                                   & E & 25                                      & \multicolumn{1}{l|}{0.44} & \multicolumn{1}{l|}{0.47} & 0.02  & \multicolumn{1}{l|}{0.49} & \multicolumn{1}{l|}{0.58} & -0.09 & \multicolumn{1}{l|}{0.43} & \multicolumn{1}{l|}{0.44} & 0.01  \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}English First \\ Language\end{tabular}}} & C & 18                                      & \multicolumn{1}{l|}{0.44} & \multicolumn{1}{l|}{0.51} & 0.07* & \multicolumn{1}{l|}{0.5}  & \multicolumn{1}{l|}{0.6}  & 0.10  & \multicolumn{1}{l|}{0.42} & \multicolumn{1}{l|}{0.48} & 0.06  \\ \cline{2-12} 
\multicolumn{1}{|c|}{}                                                                                   & E & 67                                      & \multicolumn{1}{l|}{0.47} & \multicolumn{1}{l|}{0.49} & 0.02  & \multicolumn{1}{l|}{0.57} & \multicolumn{1}{l|}{0.59} & 0.03  & \multicolumn{1}{l|}{0.45} & \multicolumn{1}{l|}{0.46} & 0.02  \\ \hline
\end{tabular}
\caption{Mean Paired Difference (in Accuracy of Clip Recognition) Among 'Unsure Students' Within Demographics with Significant Decrease in Unsurety \\ \text{*} means the paired difference was significant (<0.05 p-value in paired t-test).}
\label{table:table2}

\end{table*}

